ConTex-Human: Free-View Rendering of Human from a Single Image with Texture-Consistent Synthesis

In this work, we propose a method to address the challenge of rendering a 3D human from a single image in a free-view manner. Some existing approaches could achieve this by using generalizable pixel-aligned implicit fields to reconstruct a textured mesh of a human or by employing a 2D diffusion model as guidance with the Score Distillation Sampling (SDS) method, to lift the 2D image into 3D space. However, a generalizable implicit field often results in an over-smooth texture field, while the SDS method tends to lead to a texture-inconsistent novel view with the input image. In this paper, we introduce a texture-consistent back view synthesis module that could transfer the reference image content to the back view through depth and text-guided attention injection. Moreover, to alleviate the color distortion that occurs in the side region, we propose a visibility-aware patch consistency regularization for texture mapping and refinement combined with the synthesized back view texture. With the above techniques, we could achieve high-fidelity and texture-consistent human rendering from a single image. Experiments conducted on both real and synthetic data demonstrate the effectiveness of our method and show that our approach outperforms previous baseline methods.

==> sec/itr.tex <==
\section{Introduction}
\label{sec:intro}
% dirty, non, non, high fidelity, same style
Free-view human synthesis or rendering is essential for various applications, including virtual reality, electronic games, and movie production. Traditional approaches often require a dense camera rig or depth sensors to reconstruct the geometry and refine the texture of the subject, resulting in a tedious and time-consuming process.

% Recently, with the advent of the implicit field, remarkable progress has been made in 3D human free-view synthesis from a single RGB image. Some methods \cite{saito2019pifu, saito2020pifuhd, zheng2021pamir}, achieve this by using pixel-aligned 2D image features as input conditions for subsequent occupancy and color prediction of corresponding 3D points. They extract a mesh from the implicit field and predict the vertex color for free-view rendering. However, their rendering results exhibit over-smooth and less fine details due to the lack of novel view information and smoothness bias of implicit field. Some work\cite{huang2023one, gao2022mps, hu2023sherf} build neural radiance field from single image or multi-view images, the rendering results is also

Recently, with the advent of the implicit field, remarkable progress has been made in 3D human free-view synthesis from a single RGB image. Some methods \cite{saito2019pifu, saito2020pifuhd, zheng2021pamir}, achieve this by using pixel-aligned 2D image features as input conditions for subsequent occupancy and color prediction of corresponding 3D points. They extract a mesh from the implicit field and predict the vertex color for free-view rendering.  Some work \cite{huang2023one, gao2022mps, hu2023sherf} build neural radiance fields from single image or multi-view images. However, both rendering results exhibit over-smooth and less fine details due to the lack of novel view information and the smoothness bias of the implicit field. To forecast the invisible information, some methods \cite{qian2023magic123, melas2023realfusion, xu2023neurallift} introduce a 2D text-to-image generative model as guidance and conduct score-distillation-sampling \emph{(SDS)} to optimize a 3D representation for general object. The pipeline also works for human cases, as shown in our concurrent work \cite{huang2023tech}. Nevertheless, \emph{SDS} leads to an over-saturation and over-smooth prediction in the back view which is not texture-consistent with the input reference image, especially with not accurate text prompts. 

In this paper, we aim to achieve texture-consistent human free-view rendering with high fidelity from a single image. However, this problem is extremely challenging. We propose an innovative framework named "ConTex Human". Under this framework, we decompose our ultimate goal into two key sub-targets. The first one is how to generate a texture-consistent back view with fine details. The second one is how to paint the side and invisible region with reasonable texture region after mapping the reference and back view on the reconstructed geometry.

For back view synthesis, we are inspired by recent 2D image/video editing methods \cite{cao2023masactrl, meng2021sdedit, qi2023fatezero, wu2023tune}, which could maintain the style and texture of the original image in editing. Our key idea is to query image contents from the input reference image to generate a texture-consistent human back view through attention injection guided by text prompts. However, naively generating using only text prompts would lead to misalignment between the back view and human geometry. Therefore, we controlled this process with the depth map as guidance to ensure that the generated back view layout is well-aligned with human geometry. After mapping the reference view and back view on the geometry, we need to paint the side region and invisible region. An intuitive solution would be conducting \emph{SDS} on the given person to leverage the 2D Diffusion model prior. But \emph{SDS} only results in color distortion and over-saturation texture. To address this problem, we propose a \emph{visibility-aware patch consistency} loss to alleviate the inconsistent side view texture, which makes sure that the side and invisible region pixel value should be close to its neighbor pixels in the front or back region.

We evaluate our approach on both synthetic dataset THuman2 that has 3D textured scans as ground truth and real dataset SSHQ which includes people in various poses, clothing, and shapes. Across the experiments, our approach exhibits significant performance in both quantitative and qualitative comparisons.

In summary, this work has the following contributions:

\begin{itemize}

    \item We introduce an innovative framework called ``ConTex-Human'', which could achieve high fidelity free-view human rendering with consistent texture from single image.
    % \vspace{pt}    

    \item We design a depth and text prompt conditioned back view synthesis module that could maintain texture style and details in reference images.
    % \vspace{5pt}    
    
    \item To remove the over-saturation texture caused by \emph{SDS}, we proposed a front-back texture mapping module. A \emph{visibility-aware patch consistency} loss is also included to further alleviate the color distortion.


\end{itemize}


% To overcome these problems, in this paper, we propose an innovative framework for texture-consistent human free-view rendering with high fidelity from a single image. We are inspired by recent 2D image/video editing methods \cite{cao2023masactrl, meng2021sdedit, qi2023fatezero, wu2023tune}, which could maintain the style and texture of the original image in editing. Our key idea is to query image contents from the input reference image to generate a texture-consistent human back view through attention injection guided by text prompts and depth map. With generated 






